Kaplansky Test Problems for $R$-Modules in ZFC

Fix a ring $ R $ and look at the class of left $ R $-modules and naturally, we restrict ourselves to the case of rings such that this class is not too similar to the case $ R $ is a field. We shall solve Kaplansky test problems, all three of which say that we do not have decomposition theory, e.g., if the square of one module is isomorphic to the cube of another it does not follows that they are isomorphic. Our results are in the ordinary et theory, ZFC. For this, we look at bimodules, i.e., the structures which are simultaneously left $ R $-modules and right $ S $-modules with reasonable associativity, over a commutative ring $ T $ included in the centers of $ R $ and of $ S $. Eventually, we shall choose $ S $ to help solve each of the test questions. But first, we analyze what can be the smallest endomorphism ring of an $(R, S)$-bimodule. We construct such bimodules by using a simple version of the black box.

==> atalya.sty.tex <==
% To: "Saharon Shelah's Office" <shlhetal@math.huji.ac.il>
% Subject: ch 9 +
% Date: Tue, 15 Jul 2003 00:53:29 +0300
% From: "Atalya W.S." <Atalyah@pob.huji.ac.il>
% Mime-Version: 1.0
% X-sliced-and-diced-by: 'savemail' 1.3b, Feb 2003




\setuptheorem{Comment}


%jorej \sqrt

% Ch V: worked 1.5
\newcommand{\st}{{such that}}
\newcommand{\sq}{{sequence}}
\newcommand{\incr}{{increasing}}
\newcommand{\cont}{{continuous}}
\newcommand{\rest}{{\restriction}}
\newcommand{\rist}{{\upharpoonleft}}
\newcommand{\isom}{{isomorphism}}
\newcommand{\stati}{{stationary}}


\newcommand{\homo}{{homomorphism}}

%from Ch 3
\newcommand{\want}{{!would like}}
\newcommand{\wint}{{would like}}

\newcommand{\ppower}{{!cardinality}}
\newcommand{\power}{{cardinality}}

\newcommand{\qff}{{!quantifier free}}
\newcommand{\qqf}{{quantifier free}}


% special underline
\newcommand{\wolog}{{without loss of generality}}
\newcommand{\Wlog}{{Without loss of generality}}

\newcommand{\then}{{\underline{then}}}
\newcommand{\Then}{{\underline{Then}}}
\newcommand{\there}{{\underline{there}}}
% \newcommand{\And}{{\underline{and}}}
\newcommand{\orr}{{\underline{or}}}
\newcommand{\when}{{\underline{when}}}
\newcommand{\but}{{\underline{but}}}
\newcommand{\fsome}{{\underline{for some}}}



\newcommand{\true}{{\bf true}}
\newcommand{\false}{{\bf false}}



\newcommand{\uif}{{\underline{if}}}
\newcommand{\uIf}{{\underline{If}}}
\newcommand{\uiff}{{\underline{if and only if}}}
%\newcommand{\iff}{{if and only if}}

% new bold
\newcommand{\mymathbb}{\Bbb}

\newcommand{\bbT}{{\Bbb T}}
\setuptheorem{Main Sub Claim}
%?
%\setuptheorem{Convention}


%\usepackage{amssynb}
%\newcommand{mybbfamily}{\fontencoding{V}\fontfamily{bbold}\selectfont}
%\newcommand{\mytextbb}[1]{mybbfamily#1}}
%\DeclareMath Alyphet{\mymathbb}{V}{bbold}{m}{n}



\newcommand{\sQ}{{\mathbb Q}}
\newcommand{\cQ}{{\mymathbb Q}}
\newcommand{\cq}{{\mymathbb q}}


% NEW, Ch, unknown
\newcommand{\boll}{{\bf b}}
\newcommand{\topU}{{\dot{\cal U}}}
%= ch 12 openU

% Andrzej supplement

\setuptheorem{Main SubClaim}
\newcommand{\primp}{{\dot p}}
\newcommand{\numberisomI}{{\mathbb I}}
%\newcommand{\rinS}{{\bf S!}}
% also in ch 8
\newcommand{\sy}{{\Bbb Y}}
%[in Ch. 7]
\newcommand{\idI}{{\mathcal I}}


% Ch. 0

\newcommand{\qQ}{{\dot{\bf Q}}}
%quantifier Q

\newcommand{\setS}{{\Bbb S}}
% S(A) --- set types S

% Ch. 1

\newcommand{\bool}{{\mathbf B}}
%boolean algebra B.  +ch.4,6,7,10.

\newcommand{\blackw}{{\mathbf W}}
%black box W +4,6,7,10.

\newcommand{\FFC}{{\mathcal C}}
% ???

\newcommand{\idealI}{{\dot{\cal I}}}
%ideal I [letter i]

\newcommand{\nI}{{\Bbb I}}
% in I(\1,K) numnernonisol

\newcommand{\idJ}{{\mathcal J}}
%idealJ  cal+dot

\newcommand{\blackF}{{\mathcal F}}

\newcommand{\blackz}{{\dot \zeta}}
%[square] black box zeta. [till now bf zeta]

\newcommand{\bools}{{\dot s}}

%blackW= bf W ??
\newcommand{\blackW}{{\mathbf W}}

\newcommand{\blackZ}{{\mathbf W}}
%black box Z ???


%ideal I (Ch. 1)
\newcommand{\clubC}{{\mathcal C}}

\newcommand{\calD}{{\mathcal D}}

\newcommand{\ebool}{{\dot y}}

\newcommand{\smom}{{\mathcal M}}




%Ch. 2
% ?\newcommand{\clubC}{{\mathcal C}}

\newcommand{\const}{{\mathcal A}}
%change from clubC, only in Ch, II


%[defined ch 1]
\newcommand{\CC}{{\dot{\frak c}}}
% constr c
\newcommand{\cmuzr}{{\dot{\bf c}}}
%new

\newcommand{\ringR}{{\bf R}}
%\newcommand{\rinR}{{\bf R!}}

\newcommand{\ringr}{{\dot r}}

\newcommand{\ringS}{{\bf S}}
\newcommand{\rinS}{{\bf S!}}

\newcommand{\rings}{{\dot s}}

\newcommand{\ringT}{{\bf T}}
%\newcommand{\rinT}{{\bf T!}}

\newcommand{\ringt}{{\dot t}}

\newcommand{\ringM}{{\bf M}}


\newcommand{\ringdE}{{{dE}}}

\newcommand{\ringde}{{{de}}}

\newcommand{\ringDe}{{{De}}}

\newcommand{\ringDE}{{{D}{E}}}

\newcommand{\ringEd}{{{Ed}}}



\newcommand{\fieldD}{{{\bf D}}}



\newcommand{\moduleK}{{\mymathbb K}}
\newcommand{\modK}{{\mymathbb K}}

\newcommand{\moduleM}{{\mymathbb M}}
\newcommand{\modM}{{\mymathbb M}}

\newcommand{\moduleN}{{\mymathbb N}}
\newcommand{\modN}{{\mymathbb N}}

\newcommand{\moduleP}{{\mymathbb P}}
\newcommand{\modP}{{\mymathbb P}}

\newcommand{\moduleL}{{\mymathbb L}}
\newcommand{\modL}{{\mymathbb L}}

\newcommand{\modG}{{\mymathbb G}}


%modueequal
\newcommand{\GL}{{\Bbb G}}
%group G

%\newcommand{\primep}{{\mymathbb p}}
\newcommand{\primep}{{\dot p}}


\newcommand{\groupG}{{\Bbb G}}


\newcommand{\callE}{{\frak E}}
\newcommand{\calE}{{\frak E}}

\newcommand{\cale}{{\dot{\frak e}}}

\newcommand{\mathcallE}{{\frak E}}
%set special E

\newcommand{\callS}{{\cal S}}
%statset

\newcommand{\frakss}{{\frak m}}
%module system s

\newcommand{\sfs}{{\frak s}}
%specialtheory s
\newcommand{\sts}{{\frak t}}
%specialtheory t


\newcommand{\blackH}{{\dot{\mathbf h}}}
\newcommand{\blakH}{{\mathbf h}}

%\newcommand{\blackw}{{\mathbf W}}
%defined in Ch 1

\newcommand{\blakZ}{{\mathbf Z}}
%or dot z.
%defined means in Ch 1  bf W

\newcommand{\fucF}{{\mathbf f}}


\newcommand{\ideallI}{{\bf n}}
% ids, hds Roman

\newcommand{\isoI}{{\dot{\Bbb I}}}
%\newcommand{\isoI}{{\dot{\Bbb I!}}}
%\newcommand{\numberisomI}{{\mathbb I}}

\newcommand{\numbernonemb}{{\dot{I}\dot{E}}}
\newcommand{\numbIE}{{\dot{I}\dot{E}}}




% Ch. 3

\newcommand{\fucH}{{\mathbf h}}


\newcommand{\forG}{{\dot{\Bbb \Gamma}}}
% both turn into lneqq for unknown reason
\newcommand{\fG}{{\dot{\Bbb \Gamma}}}


\newcommand{\seqJ}{{\dot{\bf J}}}


%\newcommand{\seqI}{{\dot{\bf I}}}
\newcommand{\setI}{{\dot{\bf I}}}
\newcommand{\setId}{{\dot{\bf I}!}}



\newcommand{\Dmuzr}{{\cal D}}

\newcommand{\inve}{{\bf d}}



%number iso I

%varrho=partial

%I,IE,G,p,B,C-like before.
%L, L_{w,w,} to shadow
%sigma to vardelta.

% Ch. 4

\newcommand{\iI}{{\dot{\bf I}}}

\newcommand{\dsigma}{{\dot{\sigma}}}

%Ch. 5
\newcommand{\tT}{{T}}
%lo theory

\newcommand{\seqI}{{\dot{\bf I}}}

\newcommand{\forGa}{{\Lambda}}
%also ch 10, 11

% Ch. 6
% modG
\newcommand{\cG}{{\cal G}}

\newcommand{\seteq}{{\bf \Upsilon}}

\newcommand{\cp}{{\cal P}}

\newcommand{\fung}{{\dot G}}

\newcommand{\forceP}{{\Bbb P}}
\newcommand{\forceQ}{{\Bbb Q}}
\newcommand{\forceR}{{\Bbb R}}

% Ch. 7

% B---boolean algenra, didn't mark all.
\newcommand{\eqrelseq}{{\phi}}
\newcommand{\eqrs}{{\phi}}

\newcommand{\defeqrel}{{\phi}}

\newcommand{\funh}{{\dot{H}}}
\newcommand{\funf}{{\dot{F}}}
\newcommand{\funF}{{\dot{F}}}

\newcommand{\cc}{{\rm chain\  condition}}
%\newcommand{\Ccc}{{\dot{c}.\dot{c}.\dot{c}.}}
\newcommand{\Ccc}{{c.c.c}}
%\newcommand{\ba}{{{\rm ba}
\newcommand{\forg}{{\Lambda}}

\newcommand{\seqe}{{\bar{\bf e}}}

\newcommand{\ekxol}{{\bar{\bf e}}}


% Ch. 8
\newcommand{\bhP}{{\hat{{\Bbb P}}}}
\newcommand{\bhQ}{{\hat{{\Bbb Q}}}}
\newcommand{\bhR}{{\hat{{\Bbb R}}}}


%section 2
\newcommand{\smodule}{{\bf N}}

%[also in ch 9]
\newcommand{\forp}{{\dot{{\bf p}}}}
\newcommand{\forq}{{\dot{{\bf q}}}}
\newcommand{\forr}{{\dot{{\bf r}}}}
% forcing con r, forcingcon p...

\newcommand{\sets}{{\bf u}}
% appear in the commands list of ch 10
%\newcommand{\sett}{{\bf v}}

%small set s

\newcommand{\densd}{{\dot{{\cal D}}}}
\newcommand{\densed}{\dot{{\cal D}}}

\newcommand{\ccD}{{\dot{\Bbb D}}}


% densityfunc D

\newcommand{\dense}{{\dot{\Bbb E}}}
%density delta funcf, also Ch 9

%\newcommand{\sy}{{\cal Y}}
%set for Gamma

\newcommand{\tripr}{{\mathcal R}}
% triple R

\newcommand{\hmg}{{\rm hmg}}

%section 5

\newcommand{\forP}{{\bf P}}

\newcommand{\trivt}{{\bf t}}
% truth val t

% iddealI-cal I
% idealJ- cal J



%{ Ch. 9}

%epsilon only

%\newcommand{\vare}{\varepsilon}


%all bold D change to \hD
\newcommand{\hD}{{\hat{\bf D}}}
%densed, filterD, clubfilD

\newcommand{\Sts}{{\dot{u}}}
% every str to Sts
\newcommand{\str}{{\check{s}!}}


\newcommand{\stt}{{\dot{v}}}
% every srt change to stt
\newcommand{\srt}{{\check{t}!}}


% exist:
%ch 8: \newcommand{\sett}{{\frak v}}
%ch 8 \newcommand{\sets}{{u}}

%ch 1: \newcommand{\bools}{{\dot s}}
%ch 2: \newcommand{\rings}{{\dot s}}
%ch 2: \newcommand{\ringt}{{\dot t}}


%\underline{ Ch. 10}

\newcommand{\lo}{{\Bbb P}}

% Ch.11 [and 10]

% qQ defined Ch 1
% forGa also in 5, 10
\newcommand{\probp}{{\bf p}}
\newcommand{\setJ}{{\dot{\bf J}}}
\newcommand{\bgn}{{\Lambda}}

\newcommand{\forE}{{\dot{\epsilon}}}

\newcommand{\logbas}{{{\frak e}!}}
\newcommand{\wight}{{\dot{w}}}

\newcommand{\orderf}{{\Bbb F}}
% ? probably should cancel above
\newcommand{\ordef}{{\dot{\Bbb F}}}

% also in ch 8
\newcommand{\sett}{{\bf v}}

\newcommand{\memsets}{{\breve{f}}}
\newcommand{\memfunf}{{\dot{f}}}
\newcommand{\memfung}{{\dot{g}}}
\newcommand{\cee}{{\bf c}}
\newcommand{\funG}{{\dot G}}

\newcommand{\funH}{{\hat H}}
\newcommand{\finh}{{\hat h}}

%\newcommand{\qQ}{{\bf Q}}
%??
\newcommand{\meme}{{\dot{e}}}

\newcommand{\memn}{{\dot{n}}}
\newcommand{\memr}{{\dot{n}}}

\newcommand{\memm}{{\dot{m}}}
\newcommand{\mems}{{\dot{m}}}

\newcommand{\memk}{{\dot{k}}}
\newcommand{\meml}{{\dot{\ell}}}
\newcommand{\memh}{{\dot{h}}}

\newcommand{\memb}{{\dot{b}}}

% not in Ch 10
\newcommand{\memter}{{\dot{T}}}
% in Ch 10
\newcommand{\memt}{{\dot{k}}}

%sec 6

%+ April
\newcommand{\memtt}{{\dot{{\bf k}}}}
\newcommand{\memll}{{\dot{\ell}}}

% superscripts to \Gamma
\newcommand{\bigG}{{\mymathbb \Gamma}}
%bignessGamma
\newcommand{\bigPhi}{{\omega}}
%bignessPhi

\newcommand{\mye}{{\mymathbb e}}
%\newcommand{\ee}{{\mymathbb e}}
%\newcommand{\tS}{{\mathbb S}}
%typsetS

\newcommand{\filterD}{{\dot{D}}}
% [ch 9]
\newcommand{\clubfilD}{{\check{\cal D}}}

\newcommand{\goodI}{{\check{I}^{\rm gd}}}

\newcommand{\bb}{{b'_1}}

\newcommand{\distance}{{\dot{\bf d}}}

\newcommand{\probab}{{\bf q}}
%-----
% ??
\newcommand{\funnyD}{{Dmuzar}}

%[ XI]



%[newcommand{\bignessphi}{{\mathcal C}}]

%Ch.12
% in Ch 3 exists also as seqJ etc.

\newcommand{\wdideal}{{\check{I}^{\rm wd}}}

\newcommand{\barbI}{{\bar{\bf I}}}

\newcommand{\seqidealJ}{{\dot{\bf J}}}

\newcommand{\seqidealI}{{\dot{\bf I}}}

\newcommand{\borelB}{{\dot{\Bbb B}}}

\newcommand{\iddealI}{{\bf I}}
%already defined in Ch 1 idealI=dot cal I.



\newcommand{\idealJ}{{\bf J}}
%\newcommand{\iddealJ}{\bf J}}
% ?? \newcommand{\idealJ}{{\dot{\mathcal J}}}
%already defined in Ch 1 as idJ=cal J.

\newcommand{\openU}{{\Bbb U}}
%unclear: cal U or Bbb U. defined before on unknown list under topU

\newcommand{\fuchH}{{\dot{\bf h}}}
% fucH defined in Ch 3

\newcommand{\invee}{{\bf d}}

\newcommand{\setcard}{{\frak S}}

%pr=rpr


% Ch X, XI
\newcommand{\cll}{{c\ell}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% roman shorts in math formulas:
%%%% according to the list in intro 1

\newcommand{\racc}{{\rm acc}}

\newcommand{\racl}{{\rm acl}}

\newcommand{\ads}{{\rm ads}}

\newcommand{\AUT}{{\rm AUT}}

\newcommand{\rat}{{\rm at}}

\newcommand{\rav}{{\rm av}}

\newcommand{\BA}{{\rm BA}}

\newcommand{\rba}{{\rm ba}}

\newcommand{\rcard}{{\rm card}}

%\newcommand{\cd}{{\rm cd}}
\newcommand{\rcd}{{\rm cd}}

%\newcommand{\cf}{{\rm cf}}
\newcommand{\rcf}{{\rm cf}}

\newcommand{\rcl}{{\rm cl}}

\newcommand{\rdim}{{\rm dim}}

\newcommand{\rdis}{{\rm dis}}

\newcommand{\rDom}{{\rm Dom}}

\newcommand{\Dp}{{\rm Dp}}

\newcommand{\End}{{\rm End}}

\newcommand{\ExKer}{{\rm ExKer}}

\newcommand{\Ext}{{\rm Ext}}

\newcommand{\rGM}{{\rm GM}}

\newcommand{\hds}{{\rm hds}}

\newcommand{\rhor}{{\rm hor}}

\newcommand{\rid}{{\rm id}}

\newcommand{\rids}{{\rm ids}}

\newcommand{\rind}{{\rm ind}}

\newcommand{\rinf}{{\rm inf}}

\newcommand{\rinv}{{\rm inv}}

\newcommand{\rINV}{{\rm INV}}

\newcommand{\rbINV}{{\rm bINV}}

%\newcommand{\ris}{{\rm is}}

\newcommand{\risb}{{\rm isb}}

%\newcommand{\lg}{{\rm lg}}
% ??????
\newcommand{\rlg}{{\rm lg}}

\newcommand{\rlim}{{\rm lim}}

%default command
%\newcommand{\ln}{{\rm ln}}

%\newcommand{\log}{{\rm log}}

\newcommand{\rKer}{{\rm Ker}}

\newcommand{\mgh}{{\rm mgh}}

\newcommand{\Mod}{{\rm Mod}}

\newcommand{\rmod}{{\rm mod}}

\newcommand{\rms}{{\rm ms}}

\newcommand{\rmt}{{\rm mt}}

\newcommand{\rna}{{\rm na}}

\newcommand{\OP}{{\rm OP}}

\newcommand{\rOrd}{{\rm Ord}}

\newcommand{\PC}{{\rm PC}}

\newcommand{\rpcf}{{\rm pcf}}

\newcommand{\pk}{{\rm pk}}

\newcommand{\rpo}{{\rm po}}

\newcommand{\rpoe}{{\rm poe}}

\newcommand{\rpot}{{\rm pot}}

\newcommand{\rpp}{{\rm pp}}

\newcommand{\rpr}{{\rm pr}}

\newcommand{\rqf}{{\rm qf}}

\newcommand{\rqmt}{{\rm qmt}}

\newcommand{\rRang}{{\rm Rang}}

\newcommand{\Sp}{{\rm Sp}}

\newcommand{\rsp}{{\rm sp}}

\newcommand{\rSuc}{{\rm Suc}}

\newcommand{\Succ}{{\rm Succ}}

%\newcommand{\sup}{{\rm sup}}

\newcommand{\supp}{{\rm supp}}

\newcommand{\rTh}{{\rm Th}}

\newcommand{\rtms}{{\rm tms}}

\newcommand{\rtp}{{\rm tp}}

\newcommand{\rtr}{{\rm tr}}

\newcommand{\rRes}{{\rm Res}}

\newcommand{\ruf}{{\rm uf}}

\newcommand{\rver}{{\rm ver}}

\newcommand{\rvr}{{\rm vr}}

\newcommand{\rwm}{{\rm wm}}

\newcommand{\rwmg}{{\rm wmg}}

\newcommand{\rws}{{\rm ws}}


\newcommand{\orco}{{\rm orco}}


% old and unknown
\newcommand{\rdf}{{\rm df}}

%%% ??? What should be these??

%\newcommand{\sy}{sy}
%\newcommand{\clubC}{clubC}

%% change..
%\newcommand{\formalendsW}{{\cal W}}

\newcommand{\formalendsX}{{\cal X}}
\newcommand{\formalendsZ}{{\cal Z}}
\newcommand{\formalendsY}{{\cal Y}}



%\newcommand{\Ext}{{\rm Ext}}

